Stochastic Multivariate Universal-Radix Finite-State Machine: a Theoretically and Practically Elegant Nonlinear Function Approximator

Nonlinearities are crucial for capturing complex input-output relationships especially in deep neural networks. However, nonlinear functions often incur various hardware and compute overheads. Meanwhile, stochastic computing (SC) has emerged as a promising approach to tackle this challenge by trading output precision for hardware simplicity. To this end, this paper proposes a first-of-its-kind stochastic multivariate universal-radix finite-state machine (SMURF) that harnesses SC for hardware-simplistic multivariate nonlinear function generation at high accuracy. We present the finite-state machine (FSM) architecture for SMURF, as well as analytical derivations of sampling gate coefficients for accurately approximating generic nonlinear functions. Experiments demonstrate the superiority of SMURF, requiring only 16.07% area and 14.45% power consumption of Taylor-series approximation, and merely 2.22% area of look-up table (LUT) schemes.

==> IEEEexample.tex <==
\begin{thebibliography}{1}
\bibitem{1} Qichao Liu, Liang Xiao, Jingxiang Yang, and Zhihui Wei. Cnn-enhanced graph convolutional network with pixel and superpixel-level feature
fusion for hyperspectral image classification. IEEE Transactions on Geoscience and Remote Sensing, 59(10):8657–8671, 2021.
\bibitem{2} Qiang Zhai, Xin Li, Fan Yang, Chenglizhao Chen, Hong Cheng, and Deng-Ping Fan. Mutual graph learning for camouflaged object detection. In 2021 IEEE/CVF Conference on Computer Vision and Pattern
Recognition (CVPR), pages 12992–13002, 2021.
\bibitem{3} Rio Tomioka and Masanori Takabayashi. Dependence of activation function on image recognition accuracy in self-referential holographic
deep neural network. In 2022 Conference on Lasers and Electro-Optics Pacific Rim (CLEO-PR), pages 1–2, 2022.
\bibitem{4} Li Chai, Jun Du, Qing-Feng Liu, and Chin-Hui Lee. A cross-entropy-guided measure (cegm) for assessing speech recognition performance
and optimizing DNN-based speech enhancement. IEEE/ACM Transactions on Audio, Speech, and Language Processing, 29:106–117, 2021.
\bibitem{5} Fei Hu. Survey on neural networks in natural language processing. In 2023 IEEE International Conference on Control, Electronics and
Computer Technology (ICCECT), pages 591–594, 2023.
\bibitem{6} Zhong Meng, Sarangarajan Parthasarathy, Eric Sun, Yashesh Gaur, Naoyuki Kanda, Liang Lu, Xie Chen, Rui Zhao, Jinyu Li, and Yifan Gong. Internal language model estimation for domain-adaptive end-to-
end speech recognition. In 2021 IEEE Spoken Language Technology Workshop (SLT), pages 243–250, 2021.
\bibitem{7} Xiaowu Deng, Yuanquan Shi, Dunhong Yao, Xiyan Tang, Chunqiao Mi, Jianhua Xiao, and Xian Zhang. A kernelized support tensor-ring machine for high-dimensional data classification. In 2021 International Conference on Electronic Information Technology and Smart Agriculture (ICEITSA), pages 159–165, 2021.
\bibitem{8} Jiajun Gao, Fanzhang Li, Bangjun Wang, and Helan Liang. Unsupervised nonlinear adaptive manifold learning for global and local
information. Tsinghua Science and Technology, 26(2):163–171, 2021.
\bibitem{9} Rui Wang, Xiao-Jun Wu, and Josef Kittler. Symnet: A simple symmetric positive definite manifold deep learning method for image set classification. IEEE Transactions on Neural Networks and Learning Systems, 33(5):2208–2222, 2022.
\bibitem{10} Srujan Teja Thomdapu, Harsh Vardhan, and Ketan Rajawat. Stochastic compositional gradient descent under compositional constraints. IEEE
Transactions on Signal Processing, 71:1115–1127, 2023.
\bibitem{11} Malay K. Ganai and Franjo Ivanˇci ́c. Efficient decision procedure for non-linear arithmetic constraints using CORDIC. In 2009 Formal Methods in Computer-Aided Design, pages 61–68, 2009.
\bibitem{12} Weikang Qian and Marc D. Riedel. The synthesis of robust polynomial arithmetic with stochastic logic. In 2008 45th ACM/IEEE Design
Automation Conference, pages 648–653, 2008.
\bibitem{13} Changqing Yang and Yanyou Guo. Numerical solution of nonlinear fredholm integral equations of second kind by using hybrid of block-pulse functions and Taylor series. In 2010 IEEE International Conference on Progress in Informatics and Computing, volume 1, pages 453–455, 2010.
\bibitem{14} B.D. Brown and H.C. Card. Stochastic neural computation. i. computational elements. IEEE Transactions on Computers, 50(9):891–905, 2001.
\bibitem{15} Ramu Seva, Prashanthi Metku, Kyung Ki Kim, Yong-Bin Kim, and Minsu Choi. Approximate stochastic computing (ASC) for image processing applications. In 2016 International SoC Design Conference (ISOCC), pages 31–32, 2016.
\bibitem{16} D.K. McNeill, D. Zhao, C. Shafai, N. Chadha, A. Cuhadar, and H.C.Card. Processing noisy analog signals from microsensor arrays and VLSI
imagers using stochastic binary computations. In IEEE CCECE2002. Canadian Conference on Electrical and Computer Engineering. Conference Proceedings (Cat. No.02CH37373), volume 2, pages 986–990
vol.2, 2002.
\bibitem{17} B. R. Gaines. Stochastic Computing Systems, pages 37–172. Springer US, Boston, MA, 1969.
\bibitem{18} Xincheng Feng, Ke Hu, and Kaining Han. MM-FSM: A high-efficiency general nonlinear function generator for stochastic computation. IEEE Transactions on Computers, 71(9):1998–2009, 2022.9
\bibitem{19} Reza Hojabr, Kamyar Givaki, SM. Reza Tayaranian, Parsa Esfahanian, Ahmad Khonsari, Dara Rahmati, and M. Hassan Najafi. SkippyNN: An embedded stochastic-computing accelerator for convolutional neural networks. In 2019 56th ACM/IEEE Design Automation Conference (DAC), pages 1–6, 2019.
\bibitem{20} Eric Michael Jonas. Stochastic architectures for probabilistic computation. PhD thesis, Massachusetts Institute of Technology, 2014.
\bibitem{21} Markov A. Extension of the limit theorems of probability theory to a sum of variables connected in a chain., 1971.
\bibitem{22} S. H. Mozafari, J. J. Clark, W. J. Gross, and B. H. Meyer. Hartley
stochastic computing for convolutional neural networks. In 2021 IEEE Workshop on Signal Processing Systems (SiPS), pages 1–6, 2021.
\end{thebibliography}

==> bibtex/bib/IEEEexample.tex <==
@INPROCEEDINGS{9539267,
  author={Wu, Lan and Wang, Yuqian and Jiang, Jie and Guo, Chaoping},
  booktitle={2020 International Conference on Virtual Reality and Intelligent Systems (ICVRIS)}, 
  title={Research on the application of an improved deep convolutional neural network in image recognition}, 
  year={2020},
  volume={},
  number={},
  pages={470-472},
  keywords={Solid modeling;Image recognition;Convolution;Neural networks;Virtual reality;Feature extraction;Convolutional neural networks;convolutional neural network;image recognition;convolution kernel;information entropy},
  doi={10.1109/ICVRIS51417.2020.00118}}

@INPROCEEDINGS{9898724,
  author={Yang, Shuo},
  booktitle={2022 International Conference on Artificial Intelligence in Everything (AIE)}, 
  title={Natural Language Processing Based on Convolutional Neural Network and Semi Supervised Algorithm in Deep Learning}, 
  year={2022},
  volume={},
  number={},
  pages={174-178},
  keywords={Deep learning;Training;Supervised learning;Visual systems;Prediction algorithms;Natural language processing;Convolutional neural networks;Deep Learning;Convolutional Neural Network;Semi Supervised Algorithm;Natural Language Processing},
  doi={10.1109/AIE57029.2022.00039}}

@INPROCEEDINGS{7726292,
  author={Zuo, Lingyun and Wan, Xin and Liu, Jian},
  booktitle={2016 3rd International Conference on Information Science and Control Engineering (ICISCE)}, 
  title={Comparison of Various Neural Network Language Models in Speech Recognition}, 
  year={2016},
  volume={},
  number={},
  pages={894-898},
  keywords={Speech recognition;Error analysis;Computational modeling;Logic gates;Recurrent neural networks;Speech;neural network language model;LSTM;speech recognition;n-best lists re-score},
  doi={10.1109/ICISCE.2016.195}}

@INPROCEEDINGS{10074111,
  author={Kisanga, Patrice and Woungang, Isaac and Traore, Issa and Carvalho, Glaucio H. S.},
  booktitle={2023 International Conference on Computing, Networking and Communications (ICNC)}, 
  title={Network Anomaly Detection Using a Graph Neural Network}, 
  year={2023},
  volume={},
  number={},
  pages={61-65},
  keywords={Computational modeling;Network security;Benchmark testing;Graph neural networks;Convolutional neural networks;Computer crime;Anomaly detection;Anomaly detection;intrusion prevention system;intrusion detection systems;Activity and Event Network (AEN);Graph neural network (GNN);datasets;Graph convolutional network (GCN)},
  doi={10.1109/ICNC57223.2023.10074111}}

@INPROCEEDINGS{9862930,
  author={Gambo, Muhammad Liman and Zainal, Anazida and Kassim, Mohamad Nizam},
  booktitle={2022 International Conference on Data Science and Its Applications (ICoDSA)}, 
  title={A Convolutional Neural Network Model for Credit Card Fraud Detection}, 
  year={2022},
  volume={},
  number={},
  pages={198-202},
  keywords={Adaptation models;Adaptive systems;Data science;Credit cards;Data models;Fraud;Convolutional neural networks;credit card fraud detection;convolutional neural network;imbalanced dataset;adaptive synthetic sampling technique;online transactions},
  doi={10.1109/ICoDSA55874.2022.9862930}}

@ARTICLE{9810331,
  author={Zacchigna, Federico G.},
  journal={IEEE Embedded Systems Letters}, 
  title={Methodology for CNN Implementation in FPGA-Based Embedded Systems}, 
  year={2023},
  volume={15},
  number={2},
  pages={85-88},
  keywords={Field programmable gate arrays;Kernel;Frequency modulation;Hardware;Embedded systems;Layout;Convolutional neural networks;System-on-chip;Convolutional neural network (CNN);embedded systems;FPGA;SOC},
  doi={10.1109/LES.2022.3187382}}

@INPROCEEDINGS{8663809,
  author={Qian, Liuchen and Fu, Yuzhuo and Liu, Ting},
  booktitle={2018 IEEE 9th International Conference on Software Engineering and Service Science (ICSESS)}, 
  title={An Efficient Model Compression Method for CNN Based Object Detection}, 
  year={2018},
  volume={},
  number={},
  pages={766-769},
  keywords={Convolution;Object detection;Quantization (signal);Sensitivity;Computational modeling;Deep learning;Taylor series;Object detection;depthwise separable convolution;pruning;model compression},
  doi={10.1109/ICSESS.2018.8663809}}

@INPROCEEDINGS{8451569,
  author={Huang, Xiaosa and Wang, Shilin and Liu, Gongshen},
  booktitle={2018 25th IEEE International Conference on Image Processing (ICIP)}, 
  title={Detecting Double Jpeg Compression with Same Quantization Matrix Based on Dense Cnn Feature}, 
  year={2018},
  volume={},
  number={},
  pages={3813-3817},
  keywords={Feature extraction;Image coding;Transform coding;Quantization (signal);Q-factor;Finite wordlength effects;Computer architecture;Double JPEG compression detection;Same quantization matrix;CNN},
  doi={10.1109/ICIP.2018.8451569}}

@INPROCEEDINGS{9390687,
  author={Li, Mingyue and He, Lesheng and Lei, Chen and Gong, Youmei},
  booktitle={2021 IEEE 5th Advanced Information Technology, Electronic and Automation Control Conference (IAEAC)}, 
  title={Fine-grained image classification model based on improved SqueezeNet}, 
  year={2021},
  volume={},
  number={},
  pages={393-399},
  keywords={Visualization;Image recognition;Tensors;Memory management;Task analysis;Kernel;Image classification;Fine-grained image classification;lightweight CNN;SqueezeNet;attention mechanism;feature fusion},
  doi={10.1109/IAEAC50856.2021.9390687}}



@INPROCEEDINGS{5351140,
  author={Ganai, Malay K. and Ivančić, Franjo},
  booktitle={2009 Formal Methods in Computer-Aided Design}, 
  title={Efficient decision procedure for non-linear arithmetic constraints using CORDIC}, 
  year={2009},
  volume={},
  number={},
  pages={61-68},
  keywords={Surface-mount technology;Nonlinear control systems;Control systems;Search engines;Floating-point arithmetic;Constraint theory;National electric code;Laboratories;Numerical stability;Operations research},
  doi={10.1109/FMCAD.2009.5351140}}

@INPROCEEDINGS{4555898,
  author={Weikang Qian and Riedel, Marc D.},
  booktitle={2008 45th ACM/IEEE Design Automation Conference}, 
  title={The synthesis of robust polynomial arithmetic with stochastic logic}, 
  year={2008},
  volume={},
  number={},
  pages={648-653},
  keywords={Robustness;Polynomials;Arithmetic;Stochastic processes;Logic;Stochastic resonance;Circuits;Signal synthesis;Uncertainty;Signal processing;Stochastic Logic;Probabilistic Logic;Polynomial Arithmetic},
  doi={}}

@INPROCEEDINGS{5687585,
  author={Changqing Yang and Yanyou Guo},
  booktitle={2010 IEEE International Conference on Progress in Informatics and Computing}, 
  title={Numerical solution of nonlinear Fredholm integral equations of second kind by using hybrid of block-pulse functions and Taylor series}, 
  year={2010},
  volume={1},
  number={},
  pages={453-455},
  keywords={Approximation methods;Hybrid functions;Fredholm integral equation;Block-pulse;Taylor series;Product operation matrix;Approximation},
  doi={10.1109/PIC.2010.5687585}}

@ARTICLE{954505,
  author={Brown, B.D. and Card, H.C.},
  journal={IEEE Transactions on Computers}, 
  title={Stochastic neural computation. I. Computational elements}, 
  year={2001},
  volume={50},
  number={9},
  pages={891-905},
  keywords={Stochastic processes;Computer networks;Artificial neural networks;Circuits;Optical noise;Stochastic resonance;Performance gain;Signal generators;Character recognition;Noise level},
  doi={10.1109/12.954505}}

@INPROCEEDINGS{8645529,
  author={Xie, Yi and Deng, Chunhua and Liao, Siyu and Yuan, Bo},
  booktitle={2018 52nd Asilomar Conference on Signals, Systems, and Computers}, 
  title={Area-efficient K-Nearest Neighbor Design using Stochastic Computing}, 
  year={2018},
  volume={},
  number={},
  pages={782-786},
  keywords={Stochastic Computing;K-Nearest Neighbor;Area-efficient},
  doi={10.1109/ACSSC.2018.8645529}}

@INPROCEEDINGS{7799758,
  author={Seva, Ramu and Metku, Prashanthi and Kim, Kyung Ki and Kim, Yong-Bin and Choi, Minsu},
  booktitle={2016 International SoC Design Conference (ISOCC)}, 
  title={Approximate stochastic computing (ASC) for image processing applications}, 
  year={2016},
  volume={},
  number={},
  pages={31-32},
  keywords={Image edge detection;Clocks;Stochastic processes;Approximate computing;Transforms;Gray-scale},
  doi={10.1109/ISOCC.2016.7799758}}

@INPROCEEDINGS{1013077,
  author={McNeill, D.K. and Zhao, D. and Shafai, C. and Chadha, N. and Cuhadar, A. and Card, H.C.},
  booktitle={IEEE CCECE2002. Canadian Conference on Electrical and Computer Engineering. Conference Proceedings (Cat. No.02CH37373)}, 
  title={Processing noisy analog signals from microsensor arrays and VLSI imagers using stochastic binary computations}, 
  year={2002},
  volume={2},
  number={},
  pages={986-990 vol.2},
  keywords={Signal processing;Microsensors;Very large scale integration;Stochastic processes;Analog computers;Hardware;Biology computing;Random variables;Array signal processing;Biomedical signal processing},
  doi={10.1109/CCECE.2002.1013077}}

@Inbook{Gaines1969,
author="Gaines, B. R.",
editor="Tou, Julius T.",
title="Stochastic Computing Systems",
bookTitle="Advances in Information Systems Science: Volume 2",
year="1969",
publisher="Springer US",
address="Boston, MA",
pages="37--172",
abstract="The invention of the steam engine in the late eighteenth century made it possible to replace the muscle-power of men and animals by the motive power of machines. The invention of the stored-program digital computer during the second world war made it possible to replace the lower-level mental processes of man, such as arithmetic computation and information storage, by electronic data-processing in machines. We are now coming to the stage where it is reasonable to contemplate replacing some of the higher mental processes of man, such as the ability to recognize patterns and to learn, with similar capabilities in machines. However, we lack the ``steam engine'' or ``digital computer'' which will provide the necessary technology for learning and pattern recognition by machines.",
isbn="978-1-4899-5841-9",
doi="10.1007/978-1-4899-5841-9_2",
url="https://doi.org/10.1007/978-1-4899-5841-9_2"
}

@ARTICLE{9563231,
  author={Feng, Xincheng and Hu, Ke and Han, Kaining},
  journal={IEEE Transactions on Computers}, 
  title={MM-FSM : A High-Efficiency General Nonlinear Function Generator for Stochastic Computation}, 
  year={2022},
  volume={71},
  number={9},
  pages={1998-2009},
  keywords={Logic gates;Complexity theory;Signal processing algorithms;Hardware;Signal generators;Multiplexing;Taylor series;Stochastic computation;nonlinear function;general construtrure},
  doi={10.1109/TC.2021.3117127}}

@INPROCEEDINGS{9604984,
  author={Mozafari, S. H. and Clark, J. J. and Gross, W. J. and Meyer, B. H.},
  booktitle={2021 IEEE Workshop on Signal Processing Systems (SiPS)}, 
  title={Hartley Stochastic Computing For Convolutional Neural Networks}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  keywords={Performance evaluation;Energy consumption;Matched filters;Convolution;Frequency-domain analysis;Conferences;Hardware;Deep Learning;FPGA Design;Energy Consumption;Latency},
  doi={10.1109/SiPS52927.2021.00049}}

@ARTICLE{1676877,
  author={Hou},
  journal={IEEE Transactions on Computers}, 
  title={The Fast Hartley Transform Algorithm}, 
  year={1987},
  volume={C-36},
  number={2},
  pages={147-156},
  keywords={Discrete cosine transform;discrete Hartley transform;fast Hartley transform;fast Fourier transform;generalized Cooley-Tukey FFT;parallel processing;recursive algorithm},
  doi={10.1109/TC.1987.1676877}}

@phdthesis{jonas2014stochastic,
  title={Stochastic architectures for probabilistic computation},
  author={Jonas, Eric Michael},
  year={2014},
  school={Massachusetts Institute of Technology}
}

@INPROCEEDINGS{9676280,
  author={Goel, Sofia and Sharma, Sudhansh and Tripathi, RC},
  booktitle={2021 10th International Conference on System Modeling & Advancement in Research Trends (SMART)}, 
  title={Predicting Diabetes using CNN for Various Activation Functions: A Comparative Study}, 
  year={2021},
  volume={},
  number={},
  pages={665-669},
  keywords={Deep learning;Training;Convolution;Neural networks;Predictive models;Glucose;Diabetes;CNN;Pooling;Activation Function;Deep Learning;Diabetes},
  doi={10.1109/SMART52563.2021.9676280}}

@INPROCEEDINGS{8806970,
  author={Hojabr, Reza and Givaki, Kamyar and Tayaranian, SM. Reza and Esfahanian, Parsa and Khonsari, Ahmad and Rahmati, Dara and Najafi, M. Hassan},
  booktitle={2019 56th ACM/IEEE Design Automation Conference (DAC)}, 
  title={SkippyNN: An Embedded Stochastic-Computing Accelerator for Convolutional Neural Networks}, 
  year={2019},
  volume={},
  number={},
  pages={1-6},
  keywords={Convolution;Hardware;Computer architecture;Logic gates;Generators;Power demand;Neural networks},
  doi={}}

@INPROCEEDINGS{10432145,
  author={Tomioka, Rio and Takabayashi, Masanori},
  booktitle={2022 Conference on Lasers and Electro-Optics Pacific Rim (CLEO-PR)}, 
  title={Dependence of Activation Function on Image Recognition Accuracy in Self-Referential Holographic Deep Neural Network}, 
  year={2022},
  volume={},
  number={},
  pages={1-2},
  keywords={Training;Image recognition;Artificial neural networks;Lasers and electrooptics;Numerical simulation;Task analysis;Electro-optical waveguides},
  doi={10.1109/CLEO-PR62338.2022.10432145}}

@INPROCEEDINGS{9383515,
  author={Meng, Zhong and Parthasarathy, Sarangarajan and Sun, Eric and Gaur, Yashesh and Kanda, Naoyuki and Lu, Liang and Chen, Xie and Zhao, Rui and Li, Jinyu and Gong, Yifan},
  booktitle={2021 IEEE Spoken Language Technology Workshop (SLT)}, 
  title={Internal Language Model Estimation for Domain-Adaptive End-to-End Speech Recognition}, 
  year={2021},
  volume={},
  number={},
  pages={243-250},
  keywords={Training;Transducers;Estimation;Training data;Production;Acoustics;Task analysis;Speech recognition;language model;recurrent neural network transducer;attention-based encoder-decoder},
  doi={10.1109/SLT48900.2021.9383515}}

@ARTICLE{9258383,
  author={Chai, Li and Du, Jun and Liu, Qing-Feng and Lee, Chin-Hui},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
  title={A Cross-Entropy-Guided Measure (CEGM) for Assessing Speech Recognition Performance and Optimizing DNN-Based Speech Enhancement}, 
  year={2021},
  volume={29},
  number={},
  pages={106-117},
  keywords={Neural networks;Speech recognition;Speech enhancement;Acoustic measurements;Acoustics;Noise robustness;Optimization;Acoustic model;cross entropy;deep neural network (DNN);robust automatic speech recognition;speech enhancement},
  doi={10.1109/TASLP.2020.3036783}}

@INPROCEEDINGS{9577564,
  author={Zhai, Qiang and Li, Xin and Yang, Fan and Chen, Chenglizhao and Cheng, Hong and Fan, Deng-Ping},
  booktitle={2021 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Mutual Graph Learning for Camouflaged Object Detection}, 
  year={2021},
  volume={},
  number={},
  pages={12992-13002},
  keywords={Computer vision;Codes;Image edge detection;Object detection;Feature extraction;Cognition;Data mining},
  doi={10.1109/CVPR46437.2021.01280}}

@ARTICLE{9268479,
  author={Liu, Qichao and Xiao, Liang and Yang, Jingxiang and Wei, Zhihui},
  journal={IEEE Transactions on Geoscience and Remote Sensing}, 
  title={CNN-Enhanced Graph Convolutional Network With Pixel- and Superpixel-Level Feature Fusion for Hyperspectral Image Classification}, 
  year={2021},
  volume={59},
  number={10},
  pages={8657-8671},
  keywords={Feature extraction;Convolution;Kernel;Decoding;Training data;Deep learning;Computational modeling;Convolutional neural network (CNN);feature fusion;graph convolutional network (GCN);graph encoder and decoder;hyperspectral image (HSI) classification},
  doi={10.1109/TGRS.2020.3037361}}

@INPROCEEDINGS{9707302,
  author={Deng, Xiaowu and Shi, Yuanquan and Yao, Dunhong and Tang, Xiyan and Mi, Chunqiao and Xiao, Jianhua and Zhang, Xian},
  booktitle={2021 International Conference on Electronic Information Technology and Smart Agriculture (ICEITSA)}, 
  title={A Kernelized Support Tensor-Ring Machine for High-Dimensional Data Classification}, 
  year={2021},
  volume={},
  number={},
  pages={159-165},
  keywords={Support vector machines;Deep learning;Tensors;Design methodology;Statistical learning;Neural networks;Kernel;tensor ring;SVM;kernel technique;KSTRM;high-dimensional data},
  doi={10.1109/ICEITSA54226.2021.00039}}

@INPROCEEDINGS{9707302,
  author={Deng, Xiaowu and Shi, Yuanquan and Yao, Dunhong and Tang, Xiyan and Mi, Chunqiao and Xiao, Jianhua and Zhang, Xian},
  booktitle={2021 International Conference on Electronic Information Technology and Smart Agriculture (ICEITSA)}, 
  title={A Kernelized Support Tensor-Ring Machine for High-Dimensional Data Classification}, 
  year={2021},
  volume={},
  number={},
  pages={159-165},
  keywords={Support vector machines;Deep learning;Tensors;Design methodology;Statistical learning;Neural networks;Kernel;tensor ring;SVM;kernel technique;KSTRM;high-dimensional data},
  doi={10.1109/ICEITSA54226.2021.00039}}

@ARTICLE{9390301,
  author={Wang, Rui and Wu, Xiao-Jun and Kittler, Josef},
  journal={IEEE Transactions on Neural Networks and Learning Systems}, 
  title={SymNet: A Simple Symmetric Positive Definite Manifold Deep Learning Method for Image Set Classification}, 
  year={2022},
  volume={33},
  number={5},
  pages={2208-2222},
  keywords={Manifolds;Kernel;Deep learning;Principal component analysis;Visualization;Covariance matrices;Videos;Deep learning;image set classification;nonsingular covariance matrix;symmetric positive definite (SPD) manifold;(2-D)²principal component analysis (PCA)},
  doi={10.1109/TNNLS.2020.3044176}}

@ARTICLE{9390301,
  author={Wang, Rui and Wu, Xiao-Jun and Kittler, Josef},
  journal={IEEE Transactions on Neural Networks and Learning Systems}, 
  title={SymNet: A Simple Symmetric Positive Definite Manifold Deep Learning Method for Image Set Classification}, 
  year={2022},
  volume={33},
  number={5},
  pages={2208-2222},
  keywords={Manifolds;Kernel;Deep learning;Principal component analysis;Visualization;Covariance matrices;Videos;Deep learning;image set classification;nonsingular covariance matrix;symmetric positive definite (SPD) manifold;(2-D)²principal component analysis (PCA)},
  doi={10.1109/TNNLS.2020.3044176}}

@INPROCEEDINGS{10141113,
  author={Hu, Fei},
  booktitle={2023 IEEE International Conference on Control, Electronics and Computer Technology (ICCECT)}, 
  title={Survey on Neural Networks in Natural Language Processing}, 
  year={2023},
  volume={},
  number={},
  pages={591-594},
  keywords={Surveys;Recurrent neural networks;Computational modeling;Semantics;Dogs;Predictive models;Linguistics;Neural Network;Word Embedding;Recurrent Neural Network;Language Model},
  doi={10.1109/ICCECT57938.2023.10141113}}

@ARTICLE{9147154,
  author={Gao, Jiajun and Li, Fanzhang and Wang, Bangjun and Liang, Helan},
  journal={Tsinghua Science and Technology}, 
  title={Unsupervised nonlinear adaptive manifold learning for global and local information}, 
  year={2021},
  volume={26},
  number={2},
  pages={163-171},
  keywords={Feature extraction;Manifolds;Approximation algorithms;Topology;Data mining;Kernel;Cost function;unsupervised manifold learning;global and local information;adaptive neighbor selection method;kernel matrix},
  doi={10.26599/TST.2019.9010049}}

@ARTICLE{10048585,
  author={Thomdapu, Srujan Teja and Vardhan, Harsh and Rajawat, Ketan},
  journal={IEEE Transactions on Signal Processing}, 
  title={Stochastic Compositional Gradient Descent Under Compositional Constraints}, 
  year={2023},
  volume={71},
  number={},
  pages={1115-1127},
  keywords={Optimization;Signal processing algorithms;Random variables;Convergence;Approximation algorithms;Complexity theory;Stochastic processes;Stochastic gradient descent (SGD);stochastic compositional gradient descent (SCGD);constrained stochastic compositional gradient descent (CSCGD)},
  doi={10.1109/TSP.2023.3244326}}

@INPROCEEDINGS{8806970,
  author={Hojabr, Reza and Givaki, Kamyar and Tayaranian, SM. Reza and Esfahanian, Parsa and Khonsari, Ahmad and Rahmati, Dara and Najafi, M. Hassan},
  booktitle={2019 56th ACM/IEEE Design Automation Conference (DAC)}, 
  title={SkippyNN: An Embedded Stochastic-Computing Accelerator for Convolutional Neural Networks}, 
  year={2019},
  volume={},
  number={},
  pages={1-6},
  keywords={Convolution;Hardware;Computer architecture;Logic gates;Generators;Power demand;Neural networks},
  doi={}}

@misc{1370283694353108108,
author="A, Markov",
title="Extension of the limit theorems of probability theory to a sum of variables connected in a chain.",
journal="Dynam Probabilist Syst",
year="1971",
volume="1",
pages="552",
URL="https://cir.nii.ac.jp/crid/1370283694353108108"
}

@Inbook{Gaines1969,
author="Gaines, B. R.",
editor="Tou, Julius T.",
title="Stochastic Computing Systems",
bookTitle="Advances in Information Systems Science: Volume 2",
year="1969",
publisher="Springer US",
address="Boston, MA",
pages="37--172",
abstract="The invention of the steam engine in the late eighteenth century made it possible to replace the muscle-power of men and animals by the motive power of machines. The invention of the stored-program digital computer during the second world war made it possible to replace the lower-level mental processes of man, such as arithmetic computation and information storage, by electronic data-processing in machines. We are now coming to the stage where it is reasonable to contemplate replacing some of the higher mental processes of man, such as the ability to recognize patterns and to learn, with similar capabilities in machines. However, we lack the ``steam engine'' or ``digital computer'' which will provide the necessary technology for learning and pattern recognition by machines.",
isbn="978-1-4899-5841-9",
doi="10.1007/978-1-4899-5841-9_2",
url="https://doi.org/10.1007/978-1-4899-5841-9_2"
}

Those fields that are not to be changed can be left out.
@IEEEtranBSTCTL{IEEEexample:BSTcontrol,
  CTLuse_article_number     = "yes",
  CTLuse_paper              = "yes",
  CTLuse_forced_etal        = "no",
  CTLmax_names_forced_etal  = "10",
  CTLnames_show_etal        = "1",
  CTLuse_alt_spacing        = "yes",
  CTLalt_stretch_factor     = "4",
  CTLdash_repeated_names    = "yes",
  CTLname_format_string     = "{f.~}{vv~}{ll}{, jj}",
  CTLname_latex_cmd         = "",
  CTLname_url_prefix        = "[Online]. Available:"
}
